Imitation with Neural Density Models

We propose a new framework for Imitation Learning (IL) via density estimation of the expert's occupancy measure followed by Maximum Occupancy Entropy Reinforcement Learning (RL) using the density as a reward. Our approach maximizes a non-adversarial model-free RL objective that provably lower bounds reverse Kullback-Leibler divergence between occupancy measures of the expert and imitator. We present a practical IL algorithm, Neural Density Imitation (NDI), which obtains state-of-the-art demonstration efficiency on benchmark control tasks.

==> proofs/compatible_rl_js.tex <==
\begin{lemma}
If $\gM_x \sim \gM_y$ and $\gM^*_x$ and $\gM^*_y$ are maximal reductions to $\gM_x$ and $\gM_y$ respectively, then there exists an isomorphism between $\gM^*_x$ and $\gM^*_y$.
\end{lemma}
\begin{proof}
Since $\gM_x \sim \gM_y$, there exists $\gM^*$ such that $\gM^* \leq \gM_x$ and $\gM^* \leq \gM_y$. Therefore, there exists a maximal reduction of $\gM_x$ or $\gM_y$ that is also a reduction of $\gM^*$. The uniqueness of a maximal reduction ensures that the maximal reduction of $\gM_x$ or $\gM_y$ must be a reduction of $\gM^*$.
\end{proof}

\begin{theorem}
If $\mx \sim \my$, then if for some $f^*$ and $g^*$ such that:
$$
\pi_{x} = g \circ \pi_{y} \circ f \text{ is optimal in } \gM \quad \text{and} \quad \rho_{\pi_{x}}(\tau_{y}) = \rho_{\pi_{y}}(\tau_{y})
$$ 
then there exists $\gM^*$ such that $\gM^*$ is a maximal reduction of $\mx$ and $\my$, 
$\gM^* \leq_{\phi_x, \psi_x} \gM_x$ and $\gM^* \leq_{\phi_y, \psi_y} \gM_y$, where $f^* \in \phi_y^{-1} \circ \phi_x$ and $g^* \in \psi_x^{-1} \circ \psi_y$.
\end{theorem}
\begin{proof}
Consider the mapping from $(\gS^\star, \gA^\star)$ defined as $h^* = (\phi_y \circ f^* \circ \phi_x^{-1}, \psi_{y}^{-1} \circ g^* \circ \psi_x)$, we show this forms a valid homomorphism from $\gM^*$ to $\gM^*$.

\paragraph{Dynamics preservation} 
For all $s^* \in \gS^*$ if $a^*$ is an optimal action for $s^*$ then 

\js{todo}
As $\rho_{\pi_{x}}(\tau_{y}) = \rho_{\pi_{y}}(\tau_{y})$, $f$ has to be a surjection.

\paragraph{Reward preservation} \js{todo}

Since $\gM^*$ is a maximal reduction, there does not exist non-identity automorphisms, so $(\phi_y \circ f^* \circ \phi_x^{-1}, \psi_{y}^{-1} \circ g^* \circ \psi_x)$ defines an identity relationship:
\begin{align*}
    \phi_y \circ f^* \circ \phi_x^{-1} = I \\
    \psi_{y}^{-1} \circ g^* \circ \psi_x = I
\end{align*}

\end{proof}

==> proofs/reduction_uniqueness.tex <==
\begin{lemma} The maximal reduction $\mc{M}^*$ of an MDP $\mc{M}$ is ``unique'', i.e. all the maximal reductions are isomorphic to each other. 
\label{lemma:max_reduction}
\end{lemma}
\begin{proof}
If the maximal reduction is not unique, then $\exists \gM_1, \gM_2$ such that $\gM_1$ and $\gM_2$ are both maximal reductions of $\gM$ and that $\gM_1$ and $\gM_2$ are not equivalent. We proceed to show that we can construct a $\phi_3$ and $\psi_3$ such that the corresponding reduction is a strictly smaller reduction of $\gM_1$ and $\gM_2$, which proves the lemma by contradiction.

(Construction of $\phi_3$) For $s, s' \in \mc{S}$, we define $s$ is ``reachable'' to $s'$ if there exists a sequence $s_1, s_2, \ldots, s_{k-1}$ such that $\forall i=0, \ldots, k$, 
\begin{align}
\phi_1(s_i) = \phi_1(s_{i+1}) \quad \text{or} \quad \phi_2(s_i) = \phi_2(s_{i+1}) \quad \text{holds.} \label{eq:state12}
\end{align}
where $s_0 := s, s_{k} := s'$
The ``reachable'' relationship defines an equivalence class $[\gS_i]$ and we simply assign $\phi_3(s) = i$ if $s \in \gS_i$. 

(Verifying dynamics preservation for $\phi_3$) For all $s, s' \in \mS$ such that $\phi_3(s) = \phi_3(s')$ and corresponding $s_1, s_2, \ldots, s_{k-1}$ sequence, we have $\forall a \in \gA, i \in 0, \ldots, k$:
$$
\phi_1(T(s_{i}, a)) = \phi_1(T(s_{i+1}, a)) \quad \text{or} \quad \phi_2(T(s_{i}, a)) = \phi_2(T(s_{i+1}, a)),
$$
from the definition of dynamics preservation and Equation~\ref{eq:state12}.
Therefore $\phi_3(T(s_{i}, a)) = \phi_3(T(s_{i+1}, a))$, and so $\phi_3(T(s, a)) = \phi_3(T(s', a))$ due to transitive property of equality. 

(Construction of $\psi_3$) We repeat a similar argument for actions. We define $a$ is ``reachable'' to $a'$ if there  exists a sequence $a_1, a_2, \ldots, a_{k-1}$ such that $\forall i=0, \ldots, k$, 
\begin{align}
    \psi_1(a_i) = \psi_1(a_{i+1}) \quad \text{or} \quad \psi_2(a_i) = \psi_2(a_{i+1}) \quad \text{holds.} \label{eq:action12}
\end{align}
Again, this defines an equivalence class $[\gA_i]$ and we assign $\psi_3(a) = i$ if $a \in \gA_i$. 

(Verifying dynamics preservation for $\psi_3$) For all $a, a' \in \gA$ such that $\phi_3(a) = \phi_3(a')$ and corresponding $a_1, a_2, \ldots, a_{k-1}$ sequence, we have $\forall s \in \gS, i \in 0, \ldots, k$:
$$
\phi_1(T(s, a_{i})) = \phi_1(T(s, a_{i+1})) \quad \text{or} \quad \phi_2(T(s, a_{i})) = \phi_2(T(s, a_{i+1})),
$$
which is from the definition of dynamics preservation and Equation~\ref{eq:action12}.
Thus $\phi_3(T(s, a_{i})) = \phi_3(T(s, a_{i+1}))$ and so $\phi_3(T(s, a)) = \phi_1(T(s, a'))$ holds due to transitive property of equality. 

Moreover, for $s, s' \in \gS, a, a' \in \gA$ such that $\phi_3(s) = \phi_3(s')$ and $\psi_3(a) = \psi_3(a')$ \js{we preserve the optimal policy, will flush this out once we settle with a formalization.}

% Since $\gM_1$ and $\gM_2$ are not equivalent, so there exists some state or action where Equation~\ref{eq:state12} or~\ref{eq:action12} holds true. 
Hence $\gM_3 \leq \gM_1$ and $\gM_3 \neq \gM_1$, and this contradicts the assumption that $\gM_1$ is a minimal reduction; the same argument holds for $\gM_2$.
\end{proof}

==> sections/alignability.tex <==
\section{Alignable MDPs}
\label{section:alignability}
Let $\Pi^{*}_{\mc{M}}$ be the set of all optimal policies for MDP $\mc{M}$. We define an occupancy measure \citep{syed2008apprenticeship} $q_{\pi}: \S \times \A \rightarrow \sR$ for policy $\pi$ executed in MDP $\mc{M}$ as $q_{\pi}(s, a) = \pi(a | s) \sum_{t=0}^{\infty} \gamma^{t} \Pr(s^{(t)} = s; \pi, \mc{M})$. We further define the optimality function $O_{\mx}: \sx \times \ax \rightarrow \{0, 1\}$ for an MDP $\mx$ as $O_{\mx}(s_{x}, a_{x}) = 1$ if $\exists \pi_{x}^* \in \Pi^{*}_{\mx}$ such that $(s_{x}, a_{x}) \in \mathrm{supp}(q_{\pi_{x}^*})$ and $O_{\mx}(s_{x}, a_{x}) = 0$ otherwise. We are now ready to formalize MDP reductions: a class of structure preserving maps between MDPS. 

%%%%%%%%%%%%%%%%%%%%%% MDP REDUCTION DEFINITION %%%%%%%%%%%%%%%%%%%%%%
\begin{restatable}{definition}{mdpreduction} An \textbf{MDP reduction} from $\mx = (\sx, \ax, \px, \eta_{x}, \rx)$ to $\my = (\sy, \ay, \py, \eta_{y}, \ry)$ is a tuple $r = (\phi, \psi)$ where $\phi: \sx \to \sy, \psi: \ax \to \ay$ are maps that preserve: 
\vspace{-5pt}
\begin{enumerate}
\thinmuskip=0mu
\item ($\pi$-optimality) $\forall (s_{x}, a_{x}, s_{y}, a_{y}) \in \sx \times \ax \times \sy \times \ay:$ 
\begin{flalign}
&O_{\my}(\phi(s_{x}),\psi(a_{x})) = 1\Rightarrow O_{\mx}(s_{x},a_{x})=1&\label{eq:reward}\\
&O_{\my}(s_{y}, a_{y}) = 1 \Rightarrow \phi^{-1}(s_{y}) \neq \emptyset, \psi^{-1}(a_{y}) \neq \emptyset \label{eq:surjective} 
\end{flalign}
\vspace{-15pt}
\item (dynamics) $\forall (s_{x}, a_{x}, s_{y}, a_{y}) \in \sx \times \ax \times \sy \times \ay$ such that $O_{\my}(s_{y}, a_{y}) = 1, s_{x} \in \phi^{-1}(s_{y}), a_{x} \in \psi^{-1}(a_{y}):$ 
\begin{align}
    \py(s_{y}, a_{y}) = \phi(\px(s_{x}, a_{x})) \label{eq:transition}
\end{align}
\end{enumerate}
% \vspace{-5pt}
where we define $\phi^{-1}(s_{y}) = \{ s_{x} | \phi(s_{x}) = s_{y} \}$,  $\psi^{-1}(a_{y}) = \{ a_{x} | \psi(a_{x}) = a_{y} \}$.
Furthermore, $r$ is an \textbf{MDP permutation} if and only if $\phi, \psi$ are bijective maps.
\end{restatable}
In words, Eq. \ref{eq:reward} states that only optimal state, action pairs in $x$  can be mapped to optimal state, action pairs in $y$ and Eq.  \ref{eq:surjective} states that $r$ must be surjective on the set of optimal state, action pairs in $y$. These properties imply that a policy in $\mx$ should have more flexibility choosing optimal actions than one in $\my$. Eq. \ref{eq:transition} states that a reduction must preserve (deterministic) dynamics. We use the notation $\mx \geq_{\phi, \psi} \my$ to denote that $(\phi, \psi)$ is a reduction from $\mx$ to $\my$, and the shorthand $\mx \geq \my$ to denote that $\mx$ reduces to $\my$.
To gain an intuitive understanding of MDP reductions, picture the execution trace of an optimal policy as a directed graph with colored edges in which the nodes correspond to states visited by an optimal policy, and the colored edges correspond to actions taken. An MDP reduction from $\mx$ to $\my$ homomorphs the execution graph of an optimal policy in $\mx$ to a execution graph of an optimal policy in $\my$. Figure  \ref{fig:isomorphism} shows an example of a valid reduction from $\mx$ to $\my$: states $1, 2$ in $\sx$ are mapped (merged) to state $a$ in $\sy$ and the blue, red actions in $\ax$ are mapped to the green action in $\ay$. Intuitively, if $\mx \geq_{\phi, \psi} \my$, then $(\phi, \psi)$ compresses $\mx$ by merging all optimal state, action pairs that have identical dynamics properties.
\begin{restatable}{definition}{alignability} 
\label{def:alignability}
Two MDPs $\mx, \my$ are \textbf{alignable} if and only if $\mx \geq \my$ or $\my \geq \mx$.
\end{restatable}
\vspace{-5pt}
Definition \ref{def:alignability} states that MDPs are alignable if reductions exists between them, meaning that they share structure. We use  $\Gamma(\mx, \my) = \{(\phi, \psi) | \mx \geq_{\phi, \psi} \my\}$ to denote the set of all valid reductions from $\mx$ to $\my$. Reductions have a particularly useful property which is that they adapt policies across alignable MDPs. Consider a state map $f: \sx \rightarrow \sy$, an inverse action map $g: \ay \rightarrow \ax$, and a composite policy $\hat{\pi}_{x} = g \circ \pi_{y} \circ f$ (see Figure \ref{fig:setup}(b)). In words, $\hat{\pi}_{x}$ maps a self state to an expert state via $f$, simulates the expert’s action choice for the mapped state via $\pi_y$, then chooses a self action that corresponds to the simulated expert action with $g$. The following lemma holds for $\hat{\pi}_x$.
% \vspace{-5pt}
% \begin{wrapfigure}{r}{0.4\textwidth}
\begin{figure}[t]
% \vspace{-20pt}
  \begin{center}
    \includegraphics[width=0.45\textwidth]{figures/isomorphism_new.pdf}
  \end{center}
  \vspace{-10pt}
  \caption{\textbf{MDP Reduction Example} between execution traces in $\mx$ (Left) and $\my$ (Right), where $\mx \geq \my$. States correspond to nodes and actions to colors. The shown reduction merges nodes in dotted boxes to their corner label, e.g $\phi(1) = \phi(2) = a$, and both blue, red actions in $\mx$ to the green action in $\my$. }
  \vspace{-10pt}
  \label{fig:isomorphism} 
\end{figure}
% \end{wrapfigure}

\begin{restatable}{theorem}{piadapt}
\label{lemma:pi_adapt}
Let $\mx, \my$ be MDPs satisfying Assumption \ref{ass:regularity} (see Appendix \ref{sec:proofs}), $\mx \geq_{\phi, \psi} \my$, and $\pi_{y}$ be optimal in $\my$. Then, $\forall g: \ay \rightarrow \ax$ s.t $\psi \circ g(a_y) = a_y ~~ \forall a_{y} \in \{a_{y} | \exists s_{y} \in \sy~s.t~O_{\my}(s_{y}, a_{y}) = 1\}$, it holds that $\hat{\pi}_{x} = g \circ \pi_{y} \circ \phi$ is optimal in $\mx$.
\end{restatable}
\vspace{-5pt}
Theorem \ref{lemma:pi_adapt} states that the state, action maps $(f, g^{-1})$ chosen to be a reduction can adapt optimal policies between alignable MDPs. Here onwards we interchangeably refer to $(f, g)$ as "alignments". We now show how the DAIL problem can be solved by first solving an MDP alignment problem followed by an adaptation step. 

\begin{restatable}{definition}{compatibility}
\label{def:jointalign}
Let $(\mx, \my), (\mx', \my') \in \Omega^2$ be two MDP pairs. Then, $(\mx, \my) \sim (\mx', \my')$, i.e they are \textbf{joint alignable}, if $\Gamma(\mx, \my) \cap \Gamma(\mx', \my') \neq \emptyset$.  
\end{restatable}
\vspace{-5pt}
In words, two MDP pairs are joint alignable if there exists a shared reduction. We define an equivalence class $[(\mx, \my)]_{\sim} = \{(\mx', \my')~~|~~(\mx', \my') \sim (\mx, \my)\}$ of MDP pairs that share reductions. Overloading notation, $\Gamma(\{(\mx^{i}, \my^{i})\}_{i=1}^{N}) = \{(\phi, \psi)~|~(\phi, \psi) \in \Gamma(\mx^{1}, \mx^{1}) \cap \cdots \cap \Gamma(\mx^{N}, \mx^{N})\}$. 
We now formally state the MDP alignment problem: Let $(\mx_{, \T}, \my_{, \T})$ be an MDP pair for a target task $\T$. Given an alignment task set $\mc{D}_{x, y} = \{(\mc{D}_{\mx_{, \T_{i}}}, \mc{D}_{\my_{, \T_{i}}})\}_{i = 1}^{N}$ comprising unpaired, unaligned demonstrations for MDP pairs $\{(\mx_{, \T_{i}}, \my_{, \T_{i}})\}_{i = 1}^{N} \subseteq [(\mx_{, \T}, \my_{, \T})]_{\sim}$, determine $(\phi, \psi) \in \Gamma(\{(\mx_{, \T_{i}}, \my_{, \T_{i}})\}_{i = 1}^{N})$ such that $(\phi, \psi) \in \Gamma(\mx_{, \T}, \my_{, \T})$. As shown in Figure \ref{fig:region}, with more MDP pairs, there are likely a smaller the number of joint alignments $|\Gamma(\{(\mx_{, \T_{i}}, \my_{, \T_{i}})\}_{i = 1}^{N})|$ and, as a result, $(\phi, \psi) \in \Gamma(\{(\mx_{, \T_{i}}, \my_{, \T_{i}})\}_{i = 1}^{N})$ is more likely to "generalize" to an MDP pair for a new target task $(\mx_{, \T}, \my_{, \T})$ in the equivalence class. Analogously, in a standard supervised learning problem, more training data is likely to shrink the set of models performing optimally on the training set but poorly on the test set. We can then use $(\phi, \psi)$ for DAIL: given cross domain demonstrations $\mc{D}_{\my_{, \T}}$ for the target task $\T$, learn an expert domain policy $\pi_{y, \T}$, and adapt it into the self domain using $(\phi, \psi)$ according to Theorem \ref{lemma:pi_adapt}. 

We can now assess when domains with embodiment and viewpoint mismatch have meaningful state correspondences, i.e MDP reductions, thus allowing for domain adaptive imitation. The states of a human expert with more degrees of freedom than a robot imitator can be merged into the robot states if the task only requires the robot's degrees of freedom and the execution traces share structure, e.g traces are both cycles. However, if the task requires all degrees of freedom possessed only by the human, the robot cannot find meaningful correspondences, and also cannot imitate the task. Two MDPs for different viewpoints of an agent performing a task are MDP permutations since there is a one-to-one correspondence between state, actions at same timestep in the execution trace of an optimal policy. 


% \begin{wrapfigure}{r}{0.25\textwidth}
\begin{figure}[t]
%   \vspace{-10pt}
  \begin{center}
    \includegraphics[width=0.2\textwidth]{figures/region.png}
  \end{center}
  \vspace{-10pt}
  \caption{\textbf{MDP Alignment Problem}. Blue/red, and green regions denote sets of MDP alignments for two alignment tasks and the target task, respectively. White hatches cover the solution set to the MDP alignment problem which is the intersection of all sets}
  \vspace{-10pt}
  \label{fig:region}
\end{figure}
% \end{wrapfigure}

%%%%%%%%%% SECTION 4 %%%%%%%%%%%
\section{Learning MDP Reductions}
\label{section:discovery}
We now derive objectives that can be optimized to learn MDP reductions. We propose distribution matching and policy performance maximization. We first define the distributions to be matched. 
\begin{definition}
\label{def:co-domain-exec}
Let $\gM_x$, ${\gM_y}$ be two MDPs and $\hat{\pi}_{x} = g \circ \pi_{y} \circ f$ for $f: \gS_x \to {\gS_y}, g: {\gA_y} \to {\gA_x}$ and policy $\pi_y$. The \textbf{co-domain policy execution process} $\gP_{\hat{\pi}_{x}} = \{\hat{s}_{y}^{(t)}, \hat{a}_{y}^{(t)}\}_{t \geq 0}$ is realized by running $\hat{\pi}_{x}$ in $\mx$, i.e:   
\begin{align}
    s^{(0)}_x \sim \eta_{x},~~\hat{s}_y^{(t)} = f(s_x^{(t)}),~~ \hat{a}_y^{(t)} \sim {\pi}_y(\cdot | \hat{s}_{y}^{(t)}), \notag\\
    a_x^{(t)} = g(\hat{a}_{y}^{(t)}),~~s_{x}^{(t+1)} = \px(s_x^{(t)}, a_x^{(t)}) \quad \forall t \geq 0 \label{eq:policy}
\end{align}
\end{definition}
\vspace{-5pt}
The target distribution $\sigyy$ is over transitions uniformly sampled from execution traces of $\pi_{y}$ in $\my$ and the proxy distribution $\sigxy$ is over cross domain transitions uniformly sampled from realizations of $\mc{P}_{\hat{\pi}_{x}}$, i.e running $\hat{\pi}_{x}$ in $\mx$.
{\thickmuskip=0mu
\begin{align}
&\sigyy(s_y, a_y, s'_y) :=\notag \\
&\lim_{T \to \infty} \frac{1}{T} \sum\limits_{t=0}^{T} \Pr(s^{(t)}_y = s_y, a^{(t)}_y = a_y, s^{(t+1)}_y = s'_y; \pi_{y})\\
&\sigxy(s_y, a_y, s'_y) :=\notag\\
&\lim_{T \to \infty} \frac{1}{T} \sum\limits_{t=0}^{T} \Pr(\hat{s}_y^{(t)} = {s}_y, \hat{a}_y^{(t)} = {a}_y, \hat{s}_y^{(t+1)} = {s}'_y; \gP_{\hat{\pi}_{x}})
\end{align}}
We now propose two concrete objectives to optimize for: 1. optimality of $\hat{\pi}_{x}$, 2. $\sigxy = \sigyy$. In other words, we seek to learn $f, g$ that matches distributions over transition tuples in domain $y$ while maximizing policy performance in domain $x$. The former captures the dynamics preservation property from Eq. \ref{eq:transition} and the latter captures the optimal policy preservation property from Eq. \ref{eq:reward}, \ref{eq:surjective}. The following theorem uncovers the connection between our objectives and MDP reductions.

%%%%%%%%%%%%%%%%%%%% MAIN THEOREM %%%%%%%%%%%%%%%%%%%%%%%

\begin{restatable}{theorem}{main}
\label{thm:main}
Let $\mx, \my$ be MDPs satisfying Assumption \ref{ass:regularity} (see Supp Materials). If $\mx \geq \my$, then $\exists f: \gS_x \to \gS_y, g: \gA_y \to \gA_x$, and an optimal covering policy $\pi_y$ (see Appendix \ref{sec:proofs}) that satisfy objectives 1 and 2. Conversely, if $\exists f: \gS_x \to \gS_y$, an injective map $g: \gA_y \to \gA_x$ and an optimal covering policy $\pi_y$ satisfying objectives 1 and 2, then $\mx \geq \my$ and $\exists (\phi, \psi) \in \Gamma(\gM_x, \gM_y)$ s.t $f = \phi$ and $\psi \circ g(a_y) = a_y, \forall a_y \in \gA_y$.
\end{restatable}
\vspace{-5pt}
Theorem \ref{thm:main} states that if two MDP are alignable, then objectives 1 and 2 can be satisfied. Conversely, if 1 and 2 can be satisfied for two MDPs with state map $f$ and an injective action map $g$, then the MDPs must be alignable and all solutions $(f, g)$ are reductions. While Theorem \ref{thm:main} requires that MDPs be alignable to guarantee identifiability of solutions obtained via optimizing for objectives 1 and 2, our experiments will also run on MDPs that are "weakly" alignable, i.e. Eq. \ref{eq:reward}, \ref{eq:surjective}, \ref{eq:transition} do not hold exactly, but intuitively share structure. In the next section, we derive a simple algorithm to learn MDP reductions.



==> sections/conclusion.tex <==
\section{Discussion and future work}
\label{sec:futurework}
We've formalized Cross Domain Imitation Learning which encompasses prior work in transfer learning across embodiment \citep{Gupta2017Learning} and viewpoint differences \citep{stadie2017third, liu2018fromobs} along with a practical algorithm that can be applied to both scenarios. We now point out directions future work. Our MDP alignability theory is a first step towards formalizing possible shared structures that enable cross domain imitation. While we've shown that GAMA empirically works well even when MDPs are not perfectly alignable, upcoming works may explore relaxing the conditions for MDP alignability to develop a theory that covers an even wider range of real world MDPs. Future works may also try applying GAMA in the imitation from observations scenario, i.e actions are not available, by aligning observations with GAMA and applying methods from \cite{sermanet2018tcn, liu2018fromobs}. Finally, we hope to see future works develop principled ways design a minimal alignment task set, which is analogous to designing a minimal training set for supervised learning. 

==> sections/density.tex <==
\section{Density visualization for MADE}
\label{sec:app:density}

In Figure \ref{fig:density}, we show visualizations of the learned density model $q_{\phi}$. 

==> sections/dump.tex <==
\begin{comment}
\begin{align*}
\sum_{t = 1}^{\infty} \gamma^{t} I(s_{t}; s_{t - 1})
&\geq \sum_{t = 1}^{\infty} \gamma^{t} \E_{p_{n}(s_{t}^{i}, s_{t-1}^i)}[\frac{1}{n}\sum_{i=1}^{n} \log \frac{e^{f(s_{t}^{i}, s_{t-1}^{i})}}{\frac{1}{n}\sum_{j=1}^{n} e^{f(s_{t}^{j}, s_{t-1}^{i})}}] && \text{\cite{oord2018cpc}} \\
&= \sum_{t = 1}^{\infty} \gamma^{t} \E_{p_{t-1}^{n}(s_{t}^{1}, s_{t-1}^{1}, ..., s_{t}^{n}, s_{t-1}^{n})}[\frac{1}{n}\sum_{i=1}^{n} \log \frac{e^{f(s_{t}^{i}, s_{t-1}^{i})}}{\frac{1}{n}\sum_{j=1}^{n} e^{f(s_{t}^{j}, s_{t-1}^{i})}}] \\
&=\gamma\sum_{t = 0}^{\infty} \gamma^{t} \E_{p_{t}^{n}(s_{t+1}^{1}, s_{t}^{1}, ..., s_{t+1}^{n}, s_{t}^{n})}[\frac{1}{n}\sum_{i=1}^{n} \log \frac{e^{f(s_{t+1}^{i}, s_{t}^{i})}}{\frac{1}{n}\sum_{j=1}^{n} e^{f(s_{t+1}^{i}, s_{t}^{j})}}] \\
&= \gamma\sum_{t = 0}^{\infty} \gamma^{t} \E_{\pi^{n}}[\frac{1}{n}\sum_{i=1}^{n} \log \frac{e^{f(s_{t}^{i}, s_{t+1}^{i})}}{\frac{1}{n}\sum_{j=1}^{n} e^{f(s_{t}^{i}, s_{t+1}^{j})}}] \\
&= \gamma\E_{\pi^{n}}[\sum_{t = 0}^{\infty} \gamma^{t} \frac{1}{n}\sum_{i=1}^{n} \log \frac{e^{f(s_{t}^{i}, s_{t+1}^{i})}}{\frac{1}{n}\sum_{j=1}^{n} e^{f(s_{t}^{i}, s_{t+1}^{j})}}] \\
&= \gamma \E_{\pi^{n}}[\sum_{t = 0}^{\infty} \gamma^{t} r_t^{I}]
\end{align*}
where $r^{I}_{t} = \frac{1}{n}\sum_{i=1}^{n} \log \frac{e^{f(s_{t}^{i}, s_{t+1}^{i})}}{\frac{1}{n}\sum_{j=1}^{n} e^{f(s_{t}^{i}, s_{t+1}^{j})}}$
where $p^{n}_{t}(s_{t+1}^{1}, s_{t}^{1}, ..., s_{t+1}^{n}, s_{t}^{n}) = \prod_{i=1}^{n} p_{t}(s_{t+1}^{i}, s_{t}^{i})$ is the distribution over a size $n$ batch of state transitions sampled from $p_{t}$. Similarly, $\pi^{n}(\tau_{1}, ..., \tau_{n}) = \prod_{i}^{n} \pi(\tau_{i})$ and $\pi(\tau) = P_{0}(s_{0})\prod_{t=0}^{\infty}\pi(a_{t} | s_{t})P(s_{t+1} | s_{t}, a_{t})$. In words, $\pi_{n}$ is the distribution over a size $n$ batch of trajectories sampled by running $\pi$
\end{comment} 

Next we further lower bound the Mutual Information (MI) term using noise contrastive estimation following \cite{oord2018cpc}. For any choice of function $f$: 

\begin{align*}
\sum_{t = 1}^{\infty} \gamma^{t} I(s_{t}; s_{t - 1})
&\geq \sum_{t = 1}^{\infty} \gamma^{t} \E_{\substack{p(s_{t}, s_{t-1}) \\ q(\{\tilde{s}^{i}\}_{i=1}^{n-1})}}[\log \frac{e^{f(s_{t}, s_{t-1})}}{e^{f(s_{t}, s_{t-1})} + \sum_{i=1}^{n-1} e^{f(\tilde{s}^{i}, s_{t-1})}}] && \text{\cite{oord2018cpc}} \\
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} \E_{\substack{p(s_{t+1}, s_{t}) \\ q(\{\tilde{s}^{i}\}_{i=1}^{n-1})}}[\log \frac{e^{f(s_{t+1}, s_{t})}}{e^{f(s_{t+1}, s_{t})} + \sum_{i=1}^{n-1} e^{f(\tilde{s}^{i}, s_{t})}}] \\
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} \E_{\pi, q(\{\tilde{s}^{i}\}_{i=1}^{n-1})}[\log \frac{e^{f(s_{t+1}, s_{t})}}{e^{f(s_{t+1}, s_{t})} + \sum_{i=1}^{n-1} e^{f(\tilde{s}^{i}, s_{t})}}] \\
&= \gamma \E_{\pi}[\sum_{t = 0}^{\infty} \gamma^{t} \E_{q(\{\tilde{s}^{i}\}_{i=1}^{n-1})}[\log \frac{e^{f(s_{t+1}, s_{t})}}{e^{f(s_{t+1}, s_{t})} + \sum_{i=1}^{n-1} e^{f(\tilde{s}^{i}, s_{t})}}]] \\
&= \gamma \E_{\pi}[\sum_{t = 0}^{\infty} \gamma^{t} r^{\mathrm{NCE}}_{t}]
\end{align*}
where $q(\{\tilde{s}^{i}\}_{i=1}^{n-1})$ is a proposal noise distribution shared across all time-steps. Intuitively, $r_{t}^{\mathrm{NCE}}$ is large for states where the next state is highly predictable. The NCE bound becomes tighter as $n$ becomes larger and the optimal value for $f$ is at $f(s_{t+1}, s_{t}) = \log \frac{p(s_{t+1} | s_{t})}{p(s_{t})}$ independently of $n$. \cite{oord2018cpc}


\begin{lemma} 
\label{lem:entropy}
Assume that the dynamics are deterministic and injective. Then,
\begin{align*}
\gH(\rho_{\pi}) \geq \gamma\gH(\pi) + Constant
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\gH((1 - \gamma)\rho_{\pi}(s)) 
&= \gH((1 - \gamma)\sum_{t = 0}^{\infty} \gamma^{t} p(s_{t} = s)) \\
&\geq (1 - \gamma) \sum_{t = 0}^{\infty} \gamma^{t} \gH(s_{t}) && \text{Concavity of $\gH$} \\
&= (1 - \gamma)\Big(\gH(s_{0}) + \sum_{t = 1}^{\infty} \gamma^{t} \gH(s_{t})\Big)\\
&= (1 - \gamma)\gH(s_{0}) + (1 - \gamma)\sum_{t = 1}^{\infty} \gamma^{t} \gH(s_{t})\\
&\geq (1 - \gamma)\gH(s_{0}) + (1 - \gamma) \sum_{t = 1}^{\infty} \gamma^{t} \gH(s_{t} | s_{t-1}) && \text{Conditioning reduces entropy} \\
&= (1 - \gamma)\gH(s_{0}) + (1 - \gamma) \sum_{t = 1}^{\infty} \gamma^{t} \gH(a_{t-1} | s_{t-1}) && \text{Lemma \ref{lem:conditional}}\\
&= (1 - \gamma)\gH(s_{0}) + \gamma(1 - \gamma) \sum_{t = 0}^{\infty} \gamma^{t} \gH(a_{t} | s_{t}) \\
&= (1 - \gamma)\gH(s_{0}) + \gamma(1 - \gamma) \sum_{t = 0}^{\infty} \gamma^{t} \E_{p(s_{t}, a_{t})}[-\log p(a_{t} | s_{t})] \\
&= (1 - \gamma)\gH(s_{0}) + \gamma(1 - \gamma) \sum_{t = 0}^{\infty} \gamma^{t} \E_{\pi}[-\log p(a_{t} | s_{t})] \\
&= (1 - \gamma)\gH(s_{0}) + \gamma(1 - \gamma) \E_{\pi}[-\sum_{t = 0}^{\infty} \gamma^{t} \log \pi(a_{t} | s_{t})] \\
&= (1 - \gamma)\gH(s_{0}) + \gamma(1 - \gamma) \gH(\pi) &&\text{\ys{why? what's the def of $\pi$?}}
\end{align*}
We also have, 
\begin{align*}
\gH((1 - \gamma)\rho_{\pi}(s)) 
= (1 - \gamma) \gH(\rho_{\pi}(s)) + (1 - \gamma) \log (1 - \gamma) \\
\end{align*}
Combining the results and dividing both sides by $(1 - \gamma)$ we obtain 
\begin{align*}
\gH(\rho_{\pi}(s)) \geq \gamma \gH(\pi) + Constant
\end{align*}
\end{proof}

\newpage

\begin{assumption}
Assume that for the considered MDPs, the normalized occupancy measure $(1 - \gamma) \rho_{\pi_{E}}$ of any expert $\pi_{E}$ can be represented by an energy based model, i.e there exists a bounded, twice-differentiable function $r_{E}: \S \times \A \rightarrow \RR$ such that $\forall s, a \in \S \times \A$ it holds that $(1 - \gamma) \rho_{\pi_{E}}(s, a) = e^{r_{E}(s, a)} / \int_{\S \times \A} e^{r_{E}(s, a)} = e^{r_{E}(s, a)} / Z$. 
\end{assumption}



\begin{corollary}
\label{prop:main}
Let $r_{E}: \S \times \A \rightarrow \RR$ be an energy function s.t $(1-\gamma)\rho_{\pi_{E}}(s, a) = e^{r_{E}(s, a)} / Z$. Then, 
\begin{align*}
    -D_{\mathrm{KL}}(\rho_{\pi} || \rho_{\pi_{E}}) \geq \E_{\rho_\pi}[r_{E}(s, a)] + (1 + \gamma) \gH(\pi) + Constant
\end{align*}
\end{corollary}
\begin{proof}
\begin{align*}
-D_{\mathrm{KL}}(\rho_{\pi} || \rho_{\pi_{E}}) 
&= \sum_{s, a} \rho_{\pi}(s, a) (\log \rho_{\pi_{E}}(s, a) - \log \rho_{\pi}(s, a)) \\
&= \sum_{s, a} \rho_{\pi}(s, a) (\log e^{r_{E}(s, a)} - \log Z - \log (1 - \gamma) - \log \rho_{\pi}(s, a)) \\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] - \Big(\sum_{s, a} \rho_{\pi}(s, a) \log \rho_{\pi}(s, a)\Big) + Constant \\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] - \Big(\sum_{s, a} \rho_{\pi}(s, a) \log \frac{\rho_{\pi}(s, a)}{\rho_{\pi}(s)}\Big) - \sum_{s} \rho_{\pi}(s) \log \rho_{\pi}(s) + Constant\\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] - \Big(\sum_{s, a} \rho_{\pi}(s, a) \log \pi(a | s) \Big) - \sum_{s} \rho_{\pi}(s) \log \rho_{\pi}(s) + Constant\\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] + \gH(\pi) + \gH(\rho_{\pi}(s)) + Constant \\
&\geq \E_{\rho_{\pi}}[r_{E}(s, a)] + \gH(\pi) + \gamma \gH(\pi) + Constant && \text{Lemma} \ref{lem:conditional}\text{\ys{should be lemma 2}} \\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] + (1 + \gamma)\gH(\pi) + Constant && \text{Lemma}
\ref{lem:entropy}
\end{align*}
\end{proof}


Let $\{q_{t}(s)\}_{t \geq 0}$ be probability densities that satisfy $q_{t}(s) = p_{\theta, t}(s)$ where $p_{\theta, t:t+k}$ is the joint distribution of the random variables $\{s_{t}, ..., s_{t+k}\}$ induced by running $\pi_{\theta}$ in $\gM$. 






Recent approaches to Imitation Learning (IL) have a common theme of minimizing divergence metrics between occupancy measures of an expert and an imitator via adversarial optimization. While adversarial methods ..., they inherit undesirable optimization instabilities stemming from alternating min-max optimization. 

P1: Introduction to Imitation Learning and advantages of on-simulator approaches such as GAIL. The core goal of on-simulator RL is to minimize demonstration complexity at the cost of environment interactions.

P2: Previous approaches to on-simulator IL mostly utilize adversarial training \cite{ho2016generative, song2018multi, ke2019divergenceimitation, kostrikov2020valuedice} to exactly minimize divergences between the expert and imitator occupancy measures. Disadvantages of adversarial training: non-stationary reward function which leads to optimization instability which is exacerbated when the generator update step involves RL. This instability is especially exacerbated in high-dimensional environments. 

P3: To resolve these challenges, some recent works instead perform RL with a fixed heuristic reward function involving, for example, support estimation \cite{wang2020red} or policy disagreement \cite{brantley2020disagreement}. RL with these heuristic rewards alone are not guaranteed to recover the optimal policy and as a result they often need to add a behavioral cloning loss.

P4: We introduce a principled approximation to the distribution matching objective which results in RL with a fixed reward which involves density estimation followed by entropy regularized RL. This approach involves two challenges.

(1). Accurate density estimation \\
(2). Occupancy entropy regularization 

We address the first challenge with EBMs \cite{du2018ebm} and sliced score matching \cite{song2019sliced}. (why EBMs? why score matching instead of other approaches to train EBMs?). We address the second challenge by using state-novelty based exploration \cite{burda2018rnd} as an approximation to the occupancy entropy term \cite{lee2019marginal}. But we also show that simple MaxEntRL (which is a lower bound on the reverse KL) is empirically sufficient to recover the optimal policy. 

P5: There's a trade-off between optimizing the exact objective and optimization stability. (is there similar trade-offs in other problems?) Optimizing the exact objective with known methods requires adversarial optimization, which comes at the cost of stability. On the otherhand, optimizing a more stable objective requires approximations to the true objective. We empirically show that our approach empirically outperforms the former and advances the state of the art in demonstration complexity of IL. 




Claims of paper:

\begin{enumerate}
\item Minimizing mode collapsing divergences (e.g reverse KL, JS) is the main advantage of interacting with the environment over BC. This is not necessarily an advantage in "all" types of environments, but rather environments with specific properties.  
\begin{itemize}
\item In special cases knowledge environment dynamics allows you very efficiently infer what the true optimal behavior is. In the given example, you would need to know that the optimal policy is the max ent policy and the reward depends on state only.
\item Simple MDP is an example where GAIL will do the right thing (go to the correct goal state) but for the wrong reason (mode collapse).  
\item If reward depended on actions in the simple MDP, and from the other states, taking the red action was horrific, then GAIL would do terrible and BC would be better. 
\item mode-collapse has slightly a different interpretation in sequential domains since there are uncontrollable aspects of the data generation process, e.g initial distribution, stochastic dynamics 
\item Assuming your optimization is perfect, GAIL will do better than BC if you have a prior about whether mode collapse is good or not in your MDP. BC cannot make use of this prior since it does not exist in the space of policies. (there's no distribution over policy parameters that mode collapse) 
\item Another "practical" reason why GAIL would do better than BC is due to compounding error when optimization is imperfect, e.g if BC has small errors (even on the training set) then that can lead to catastrophic outcomes although BC loss is small. This is because the true density of the imitator is not evaluated.
\item Another key practical reason why GAIL does well, is because of the "done" signal from the environments. This is basically having access to "part" of the true reward function. 
\end{itemize}

\item Most SoTA IL algorithms minimize mode collapsing divergences by alternating between a sample-based estimation of the divergence followed by a generator update step which amounts to adversarial training.

\item We could instead, perform density estimation of expert occupancy followed by state marginal entropy regularized RL which amounts to minimizing reverse KL divergence. This is optimizing the same objective as AIRL. The only difference being the method of optimization. 
\begin{itemize}
\item The supervised learning analogy is the following. You have a generator trying to learn a gaussian only from samples. You could do this by minimizing JS divergence through GAN like training, or you could fit a density model on the samples, backpropagate through the density model to train the generator while adding entropy regularization. 
\item The latter is generally not a good idea because in non-sequential domains since (1). density estimation is hard with a flexible model class (2). adversarial training isn't that unstable in non-sequential settings (3). entropy regularization on the generator is difficult to do. And entropy regularization is absolutely necessary in the supervised setting or else the generator will only sample the maximum probability datapoint. Adversarial training gets around this since the discriminator doesn't let the generator only exploit one point. 
\item However, we argue that the latter is a good idea in the sequential setting. (1). we've made good progress on density estimation with flexible models, in particular EBMs (2). adversarial training can be terribly unstable when interlaced with RL (3). the strong dependence on entropy regularization can be relaxed in the MDP setting. This is because the dynamics prevents the generator from only generating one particular data point. 
\item Alternatively, we could argue that causal entropy regularized RL with the expert energy is a lower bound to negative KL divergence between occupancy measures. (in the case of discrete state spaces)  
\end{itemize}

\item Density estimation has crucial advantages over adversarial training: 
\begin{itemize}
\item Less optimization instability -> especially important for MDPs with high-dimensional state spaces, e.g images 
\item Easy to enforce priors about optimal behavior.
\end{itemize}

\item So what is the story?
\begin{itemize}

\item optimizing mode collapsing divergence is good in many realistic MDPs, which is why one should prefer GAIL over BC. 

\item However, adversarial optimization is not stable and thus hurts demonstration complexity. 

\item we propose density estimation IL optimizes the exact same mode collapsing divergence, but has two practical advantages: stability in optimization and prior enforcement. 

\item our approach is possible due to (1). progress in unnormalized density estimation with EBM of high dimensional data (2). In MDPs, state marginal entropy is highly correlated with action entropy.  

\item due to stability in optimization and prior enforcement, our method achieves state of the art demonstration complexity 

\end{itemize}


\end{enumerate}


Outline
\begin{enumerate}
\item preamble: introduction to MDPs and distribution matching IL. 
\begin{itemize}
\item infinite horizon discounted MDPs 
\item a distribution matching perspective on IL. write KL objective
\item explain how adversarial training can be used to optimize this objective, but we want to avoid it due to optimization instability. (cite GAIL, AIRL paper)
\item explain the density estimation approach involving density estimation + entropy regularization on the occupancy measure. 
\item Make explicit what the two key challenges to the density estimation approach are. (1). accurately estimating $\log \rho_{\pi_{E}}$ is tricky especially in high dimensional spaces. 
\item (2). maximizing entropy of the implicit distribution $\rho_{\pi}$. Emphasize how $\rho_{\pi}$ is an implicit distribution induced by running policy in the environment, and similar to how entropy regularization in GANs is non-trivial, this problem is tricky. 
\end{itemize}
\item section 2.1 : density estimation - EBM + score matching / MADE
\begin{itemize}
    \item EBM: define density model. give sliced score matching formula 
    \item MADE: define density model in autoregressive form. briefly describe MADE objective (max likelihood) 
    \item explain how these span two different families of models (EBM vs autogregressive) and also two different families of objectives (fisher divergence vs KL divergence)
\end{itemize}
\item section 2.2 : occupancy entropy maximization via lower bound 
\begin{itemize}
    \item lemma : occupancy entropy lower bound
    \item theorem 1 : DKL lowerbound
\end{itemize}
\end{enumerate}




\begin{lemma} 
\label{lem:entropy}
Assume that the dynamics are deterministic and injective. Let $\{q_{t}(s)\}_{t \geq 0}$ be densities that satisfy $q_{t}(s) = p_{\theta, t}(s)~\forall t \geq 0$ where $p_{\theta, t:t+k}$ is the joint distribution of $(s_{t}, ..., s_{t+k})$. Then,
\begin{align*}
\gH(\rho_{\pi_{\theta}}(s)) \geq \gamma \gH(\pi_{\theta}) + \gamma \E_{\pi_{\theta}}[\sum_{t = 0}^{\infty} \gamma^{t} r_{\mathrm{MI}}(s_{t}, a_{t}, s_{t+1})] + Constant
\end{align*}
where
\begin{align*}
    r_{\mathrm{MI}}(s_{t}, a_{t}, s_{t+1}) = f(s_{t}, s_{t+1}) -  \frac{1}{e}\big(\E_{q_{t}(\tilde{s}_{t})}[e^{f(s_{t+1}, \tilde{s}_{t})}] + \E_{q_{t+1}(\tilde{s}_{t+1})}[e^{f(\tilde{s}_{t+1}, s_{t})}]\big)
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\gH((1 - \gamma)\rho_{\pi_{\theta}}(s)) 
&= \gH((1 - \gamma)\sum_{t = 0}^{\infty} \gamma^{t} p(s_{t} = s)) \\
&\geq (1 - \gamma) \sum_{t = 0}^{\infty} \gamma^{t} \gH(s_{t}) && \text{Concavity of $\gH$} \\
&= (1 - \gamma)\Big(\gH(s_{0}) + \sum_{t = 1}^{\infty} \gamma^{t} \gH(s_{t})\Big)\\
&= (1 - \gamma)\gH(s_{0}) 
+ (1 - \gamma) \sum_{t = 1}^{\infty} \gamma^{t} \gH(s_{t} | s_{t-1}) 
+ (1 - \gamma) \sum_{t = 1}^{\infty} \gamma^{t} I(s_{t}; s_{t - 1})\\
\end{align*}
Let us consider each term separately starting with the entropy term: 
\begin{align*}
\sum_{t = 1}^{\infty} \gamma^{t} \gH(s_{t} | s_{t-1})
&= \sum_{t = 1}^{\infty} \gamma^{t} \gH(a_{t-1} | s_{t-1}) && \text{Lemma \ref{lem:conditional}}\\
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} \gH(a_{t} | s_{t}) \\
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} \E_{p(s_{t}, a_{t})}[-\log p(a_{t} | s_{t})] \\
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} \E_{\pi_{\theta}}[-\log p(a_{t} | s_{t})] \\
&= \gamma \E_{\pi_{\theta}}[-\sum_{t = 0}^{\infty} \gamma^{t} \log \pi_{\theta}(a_{t} | s_{t})] \\
&= \gamma \gH(\pi_{\theta}) 
\end{align*}

Next we further lower bound the Mutual Information (MI) term using the bound of Nguyen, Wainright, and Jordan, which we denote $I_{\mathrm{NWJ}}$. For any choice of critic function $f$, it holds that: 
\begin{align*}
I(X; Y) \geq I_{\mathrm{NWJ}} := \E_{p(x, y)}[f(x, y)] - e^{-1}\E_{p(x)}[\E_{p(y)}[e^{f(x, y)}]]
\end{align*}
Applying this, we obtain 
\begin{align*}
\sum_{t = 1}^{\infty} \gamma^{t} I(s_{t}; s_{t - 1})
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} I(s_{t+1}; s_{t}) \\
&\geq I_{\mathrm{NWJ}} := \gamma \sum_{t = 0}^{\infty} \gamma^{t} \Big(\E_{p_{\theta, t:t+1}(s_{t+1}, s_{t})}[f(s_{t+1}, s_{t})] - e^{-1}\E_{s_{t+1} \sim p_{\theta, t+1}(s_{t+1})}[\E_{\tilde{s}_{t} \sim p_{\theta, t}(s_{t})}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \Big) \\
&= \gamma \sum_{t = 0}^{\infty} \gamma^{t} \Big(\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[f(s_{t+1}, s_{t})] - e^{-1}\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \Big) \\
&= \gamma \Big(\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\sum_{t = 0}^{\infty} \gamma^{t} f(s_{t+1}, s_{t})] - e^{-1}\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \Big) \numberthis \label{eq:mi1}
\end{align*}

The first term is a discounted model-free RL objective with $r(s_{t}, a_{t}, s_{t+1} = f(s_{t+1}, s_{t})$ as the fixed reward function. The second term is not yet an RL objective since the inner expectation explicitly depends on $\theta$. We take the gradient of the second term w.r.t $\theta$: 

\begin{align*}
\nabla_{\theta} &\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]]  \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&\quad\quad+\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\nabla_{\theta} \sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&\quad\quad+\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\nabla_{\theta} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[\sum_{t = 0}^{\infty} \gamma^{t} e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&\quad\quad+\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(\tilde{a}_{t} | \tilde{s}_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&\quad\quad+\E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[\E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(\tilde{a}_{t} | \tilde{s}_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&\quad\quad+\E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(\tilde{a}_{t} | \tilde{s}_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}]] \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \Big(\E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(s_{t+1}, \tilde{s}_{t})}] + \E_{\tilde{s}_{0}, \tilde{a}_{0}, ... \sim \pi_{\theta}}[e^{f(\tilde{s}_{t+1}, s_{t})}]\Big)] \\
&= \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\Big(\sum_{t = 0}^{\infty} \nabla_{\theta} \log \pi_{\theta}(a_{t} | s_{t})\Big) \sum_{t = 0}^{\infty} \gamma^{t} \Big(\E_{\tilde{s}_{t} \sim p_{\theta, t}}[e^{f(s_{t+1}, \tilde{s}_{t})}] + \E_{\tilde{s}_{t+1} \sim p_{\theta, t+1}}[e^{f(\tilde{s}_{t+1}, s_{t})}]\Big)]
\\
&= \nabla_{\theta} \E_{s_{0}, a_{0}, ... \sim \pi_{\theta}}[\sum_{t = 0}^{\infty} \gamma^{t} \Big(\E_{q_{t}(\tilde{s}_{t})}[e^{f(s_{t+1}, \tilde{s}_{t})}] + \E_{q_{t+1}(\tilde{s}_{t+1})}[e^{f(\tilde{s}_{t+1}, s_{t})}]\Big)] \numberthis \label{eq:mi2}\\
\end{align*}

Combining the results of Eq. \ref{eq:mi1} and Eq. \ref{eq:mi2}, we see that maximizing $I_{\mathrm{NWJ}}$ is equivalent to maximizing a $\gamma$-discounted model-free RL objective with the reward set to: 
\begin{align*}
    r_{\textrm{MI}}(s_{t}, a_{t}, s_{t+1}) = f(s_{t}, s_{t+1}) -  \frac{1}{e}\big(\E_{q_{t}(\tilde{s}_{t})}[e^{f(s_{t+1}, \tilde{s}_{t})}] + \E_{q_{t+1}(\tilde{s}_{t+1})}[e^{f(\tilde{s}_{t+1}, s_{t})}]\big)
\end{align*}
Thus, 
\begin{align*}
\sum_{t = 1}^{\infty} \gamma^{t} I(s_{t}; s_{t - 1}) \geq \gamma \E_{\pi_{\theta}}[\sum_{t=0}^{\infty} r_{\textrm{MI}}(s_{t}, a_{t}, s_{t+1})] + Constant
\end{align*}

We also have, 
\begin{align*}
\gH((1 - \gamma)\rho_{\pi}(s)) 
= (1 - \gamma) \gH(\rho_{\pi}(s)) + (1 - \gamma) \log (1 - \gamma) \\
\end{align*}
Combining all the results and dividing both sides by $(1 - \gamma)$ we obtain 
\begin{align*}
\gH(\rho_{\pi}(s)) \geq \gamma \gH(\pi) + \gamma \E_{\pi}[\sum_{t = 0}^{\infty} \gamma^{t} r_{\mathrm{MI}}(s_{t}, a_{t}, s_{t+1})] + Constant
\end{align*}
and we have: 


\end{proof}


\begin{theorem}
\label{prop:main}
Let $r_{\mathrm{MI}}(s_{t}, a_{t}, s_{t+1}) = f(s_{t}, s_{t+1}) -  \frac{1}{e}\big(\E_{q_{t}(\tilde{s}_{t})}[e^{f(s_{t+1}, \tilde{s}_{t})}] + \E_{q_{t+1}(\tilde{s}_{t+1})}[e^{f(\tilde{s}_{t+1}, s_{t})}]\big)$ and $r_{E} = \log \rho_{\pi_{E}}$. Then, 
\begin{align*}
    -D_{\mathrm{KL}}(\rho_{\pi} || \rho_{\pi_{E}}) \geq J(\pi, \bar{r}=r_{E}+\gamma r_{\mathrm{MI}}) + (1 + \gamma) \gH(\pi) + Constant
\end{align*}
\end{theorem}
\begin{comment}
\begin{proof}
\begin{align*}
-D_{\mathrm{KL}}(\rho_{\pi} || \rho_{\pi_{E}}) 
&= \sum_{s, a} \rho_{\pi}(s, a) (\log \rho_{\pi_{E}}(s, a) - \log \rho_{\pi}(s, a)) \\
&= \sum_{s, a} \rho_{\pi}(s, a) (\log e^{r_{E}(s, a)} - \log Z - \log (1 - \gamma) - \log \rho_{\pi}(s, a)) \\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] - \Big(\sum_{s, a} \rho_{\pi}(s, a) \log \rho_{\pi}(s, a)\Big) + Constant \\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] - \Big(\sum_{s, a} \rho_{\pi}(s, a) \log \frac{\rho_{\pi}(s, a)}{\rho_{\pi}(s)}\Big) - \sum_{s} \rho_{\pi}(s) \log \rho_{\pi}(s) + Constant\\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] - \Big(\sum_{s, a} \rho_{\pi}(s, a) \log \pi(a | s) \Big) - \sum_{s} \rho_{\pi}(s) \log \rho_{\pi}(s) + Constant\\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] + \gH(\pi) + \gH(\rho_{\pi}(s)) + Constant \\
&\geq \E_{\rho_{\pi}}[r_{E}(s, a)] + \gH(\pi) + \gamma \gH(\pi) + \gamma \gH(\pi) Constant && \text{Lemma} \ref{lem:conditional} \\
&= \E_{\rho_{\pi}}[r_{E}(s, a)] + (1 + \gamma)\gH(\pi) + Constant && \text{Lemma}
\ref{lem:entropy}
\end{align*}
\end{proof}
\end{comment}


\begin{align*}
\gH(s_{t} | s_{t-1}) 
&= \E_{s_{t}, s_{t-1}}[-\log p(s_{t} | s_{t-1})] \\
&= -\sum_{s_{t}, s_{t-1}} p(s_{t}, s_{t-1}) \log p(s_{t} | s_{t-1}) \\
&= -\sum_{s_{t}, s_{t-1}} p(s_{t}, s_{t-1}) \log p(s_{t} | s_{t-1}) \\
&= -\sum_{s_{t}, s_{t-1}} \sum_{a_{t-1}} p(s_{t}, s_{t-1}, a_{t-1}) \log p(s_{t} | s_{t-1}) \\
&= -\sum_{s_{t}, s_{t-1}} \sum_{a_{t-1}} p(s_{t} | s_{t-1}, a_{t-1}) p(a_{t-1}, s_{t-1}) \log p(s_{t} | s_{t-1}) \\
&= -\sum_{s_{t-1}, a_{t-1}} p(a_{t-1}, s_{t-1}) \sum_{s_{t}} p(s_{t} | s_{t-1}, a_{t-1}) \log p(s_{t} | s_{t-1}) \\
&= -\sum_{s_{t-1}, a_{t-1}} p(a_{t-1}, s_{t-1}) \sum_{s_{t}} p(s_{t} | s_{t-1}, a_{t-1}) \log \sum_{a_{t-1}'} p(s_{t} | s_{t-1}, a_{t-1}') p(a_{t-1}' | s_{t-1}) \\
&= -\sum_{s_{t-1}, a_{t-1}} p(a_{t-1}, s_{t-1}) \log p(a_{t-1} | s_{t-1}) \\
&= \gH(a_{t-1} | s_{t-1})
\end{align*}









==> sections/related.tex <==
\section{Related Work}

Imitation learning (IL) approaches that address learning in the absence of an interactive oracle has revolved around behavioral cloning \cite{pomerleau1991efficient} and distribution matching \cite{ho2016generative, song2018multi}. In the conventional IL setting, demonstrations are assumed to be sampled from an expert domain equivalent to the self domain. To our knowledge, no previous work has formalized the cross domain imitation learning problem in which demonstrations are sampled from a (potentially) distinct MDP. 

Within the field of reinforcement learning (RL), transfer learning \cite{Taylor2009TransferSurvey}  between MDPs with identical state action spaces but different dynamics, has been explored in Atari games \cite{Rusu2016Progressive, Gamrian2018ImagetoImage} and sim-to-real transfer in robotics \cite{Tan2016SimtoReal}. A closely related field of cross domain transfer learning in the context of RL has explored approaches to find inter-state maps to exploit cross domain trajectories in a pretraining procedure that hopes to accelerate learning on a new task for which the reward function is available. Early works have hand-designed state maps \cite{Ammar2011SubspaceRL} or value function mappings \cite{taylor2007cross}. Canonical Correlation Analysis (CCA) \cite{Hotelling1936CCA} finds invertible projections into a basis in which the data from different domains are maximally correlated. These projections can then be composed to obtain a direct correspondence map between states. More recent works \cite{Ammar2015Unsupervised, Joshi2018Target} have utilized an unsupervised manifold alignment (UMA) algorithm which assumes the existence of hand crafted features along with a distance metric between them, then finds a linear map between states with similar local geometric properties. Instead of learning direct state maps, [1] assumes meaningful state pairings can be found via time alignment and instead focus on learning a domain invariant feature space. In contrast to this family of prior work, our approach exploits the latent structure of behaviors to learn both state, action maps in an unsupervised manner and considers the setting where reward function on the transfer task is unavailable. While we evaluate the usefulness of our learned MDP alignment maps as pretrained weights for comparison to prior work, we fundamentally desire to learn an optimal policy solely from cross domain demonstrations. 

Related to our proposed notion of MDP reductions, MDP homomorphisms \cite{Ranvindran2002Homo} have been explored with the aim of compressing state, action spaces to facilitate planning. With similar goals in mind, related works have proposed MDP similarity metrics based on bisimulation methods \cite{Ferns2004Bisumulation} and boltmzman machine reconstruction error \cite{Ammar2014Automated}. While conceptually related, these works have not proposed scalable procedures to discover the homomorphisms and have not drawn connections to cross domain learning. 



